Looking Inside Out: Anticipating Driver Intent From Videos

Anticipating driver intention is an important task when vehicles of mixed and varying levels of human/machine autonomy share roadways. Driver intention can be leveraged to improve road safety, such as warning surrounding vehicles in the event the driver is attempting a dangerous maneuver. In this work, we propose a novel method of utilizing in-cabin and external camera data to improve state-of-the-art (SOTA) performance in predicting future driver actions. Compared to existing methods, our approach explicitly extracts object and road-level features from external camera data, which we demonstrate are important features for predicting driver intention. Using our handcrafted features as inputs for both a transformer and an LSTM-based architecture, we empirically show that jointly utilizing in-cabin and external features improves performance compared to using in-cabin features alone. Furthermore, our models predict driver maneuvers more accurately and earlier than existing approaches, with an accuracy of 87.5% and an average prediction time of 4.35 seconds before the maneuver takes place. We release our model configurations and training scripts on https://github.com/ykung83/Driver-Intent-Prediction

==> framework.tex <==
\section{Introduction}

Overview of the content of this paper:

The main point of this paper is to enforce the notion that we have used the available information better than the two other most recent and state-of-the-art papers (Khairdoost et al), (Gebert et al). 

In the comparison with Khairdoost et al, we can easily compare the usage of ocular-cephalon data. They split the available FOV of the driver into 6 non-overlapping sections and use the output from their gaze-detection algorithm to map to one of the six sections which is then fed into their ML algorithm. In contrast, we map the gaze of the driver to an x-y coordinate which is then fed into the ML algorithm. This provides more nuanced information and better understanding of eye movement type (fixation, saccade, smooth pursuit, scanpath, etc) (reference Kar et al). 

In comparison with Gebert et al, we make the argument that our approach is more direct. Their approach relies on a combination of a very large CNN to figure out where the driver is looking and subsequently what maneuver is being attempted. If taking a variable length video, the output needs to be further fed through an LSTM. In contrast, our approach naturally can accept varying length time sequences, and has a dedicated algorithm figuring out the gaze direction. 

Both papers have accuracy around 83 percent so we are much better at 90. 

(Arthur add additional thoughts for external camera)

Paper layout and structure:

Abstract: enforce the idea that we are using the available data better - gaze information is very important, more precise measurements and more time-dependent analysis results in better performance

Introduction: 
\begin{itemize}
    \item the reasoning of why this is important
    \item cover the current state of the art and methods used (mainly focus on two reference papers)
    \item cover rationale of using information better - several papers cover the intricacies of eye movement and gaze + papers that correlate ocular-cephalo data with driver intention
\end{itemize}

Interior:
\begin{itemize}
    \item Go through the math on getting gaze output
    \item Go through the result of gaze algorithm and how it fits into the DL Network
    \item Provide figures showing the gaze for each driving manuever (the graphs look pretty similar, purpose is to show that without attention to small changes, it would be difficult to predict)
\end{itemize}

Exterior:
\begin{itemize}
    \item Go through the process of getting the output
    \item Go through the result of gaze algorithm and how it fits into the DL Network
    \item Provide figures showing the exterior data for each driving maneuver
\end{itemize}

DL networks integration:
\begin{itemize}
    \item Go through the different dl networks and math behind them
    \item how all the information is fed into the network
    \item Provide figures showing the breakdown of the networks
\end{itemize}

Results and comparison:
\begin{itemize}
    \item Go through how the result is calculated
    \item present the results of the different DL networks trained and tested on 1. only gaze and 2. everything
    \item Provide an explanation of the results with corresponding figures for support
    \item compare these results with state of the art 
\end{itemize}

Conclusion and future work:
\begin{itemize}
    \item reinforce that we got a better result using the same dataset because of better info usage
    \item mention future works of having 'user profiles' that inform the network about user habits to further improve accuracy 
\end{itemize}
